New accessibility measures based on unconventional big data sources

In health econometric studies we are often interested in quantifying aspects related to the accessibility to medical infrastructures. The increasing availability of data automatically collected through unconventional sources (such as webscraping, crowdsourcing or internet of things) recently opened previously unconceivable opportunities to researchers interested in measuring accessibility and to use it as a tool for real-time monitoring, surveillance and health policies definition. This paper contributes to this strand of literature proposing new accessibility measures that can be continuously feeded by automatic data collection. We present new measures of accessibility and we illustrate their use to study the territorial impact of supply-side shocks of health facilities. We also illustrate the potential of our proposal with a case study based on a huge set of data (related to the Emergency Departments in Milan, Italy) that have been webscraped for the purpose of this paper every 5 minutes since November 2021 to March 2022, amounting to approximately 5 million observations.

==> assets/dynamics.tex <==

\section{Dynamics}

Due to the increased availability of dynamic data, as a direct result of real time Electronic Patient Records and newer techniques of acquiring these data (i.e. web scraping), further dimensions might also be included into analyses. As a matter of fact the accessibility research can be partitioned into two streams, each of which accounts for different dynamic effects: multimodal spatial accessibility and temporal dynamics in spatial accessibility.
Morevover some people-based accessibility studies account for both, taking advantage of diverse movement velocities and finer space and time granularities \citep{miller_1991_modelling, kwan_2010_spacetime}. However they have been demonstrated to be ineffective for policymaking usage \citep{neutens_2015_accessibility}.
First, multimodal research \citep{lin_2018_a, mao2013measuring} solves for the the usage or preference of different means of transportation, such as public transportation, bicycles, walks, and private vehicles. These studies intended to reflect the varying journey distances or speeds of each form of transportation and their influence on the metrics.
Second, a few studies addressed the temporal variations (i.e. across time) of spatial accessibility measures \citep{jamtsho_2015_spatiotemporal, moyagmez_2018_the}. The bulk of them used the increased granularity of space and time to study how spatial accessibility varies over diverse hours frames ( \citep{hu_2019_measuring, lee_2018_utilizing, xia_2019_measuring} as in figure \ref{fig:dynamics_in_time}. Because the inputs to spatial accessibility assessments (supply, demand, and mobility) change over time \citep{xu_2015_transit}, temporal dynamics were generated using input qualities such as operation hours.

\newpage
